FewUser: Few-Shot Social User Geolocation via Contrastive Learning

To address the challenges of scarcity in geotagged data for social user geolocation, we propose FewUser, a novel framework for Few-shot social User geolocation. We incorporate a contrastive learning strategy between users and locations to improve geolocation performance with no or limited training data. FewUser features a user representation module that harnesses a pre-trained language model (PLM) and a user encoder to process and fuse diverse social media inputs effectively. To bridge the gap between PLM's knowledge and geographical data, we introduce a geographical prompting module with hard, soft, and semi-soft prompts, to enhance the encoding of location information. Contrastive learning is implemented through a contrastive loss and a matching loss, complemented by a hard negative mining strategy to refine the learning process. We construct two datasets TwiU and FliU, containing richer metadata than existing benchmarks, to evaluate FewUser and the extensive experiments demonstrate that FewUser significantly outperforms state-of-the-art methods in both zero-shot and various few-shot settings, achieving absolute improvements of 26.95\% and \textbf{41.62\%} on TwiU and FliU, respectively, with only one training sample per class. We further conduct a comprehensive analysis to investigate the impact of user representation on geolocation performance and the effectiveness of FewUser's components, offering valuable insights for future research in this area.

==> pkdd2024-long.tex <==
@inproceedings{koudounas2023barhotti,
  title={ba$\rho$tti at GeoLingIt: Beyond Boundaries, Enhancing Geolocation Prediction and Dialect Classification on Social Media in Italy},
  author={Koudounas, Alkis and Giobergia, Flavio and Benedetto, Irene and Monaco, Simone and Cagliero, Luca and Apiletti, Daniele and Baralis, Elena and others},
  booktitle={CEUR Workshop Proceedings},
  year={2023}
}

@article{lucas2022detecting,
  title={Detecting and locating trending places using multimodal social network data},
  author={Lucas, Luis and Tom{\'a}s, David and Garcia-Rodriguez, Jose},
  journal={Multimedia Tools and Applications},
  pages={1--20},
  year={2022},
  publisher={Springer}
}

@inproceedings{tai2023ripgeo,
  title={RIPGeo: Robust Street-Level IP Geolocation},
  author={Tai, Wenxin and Chen, Bin and Zhong, Ting and Wang, Yong and Chen, Kai and Zhou, Fan},
  booktitle={2023 24th IEEE International Conference on Mobile Data Management (MDM)},
  pages={138--147},
  year={2023}
}

@INPROCEEDINGS{matsumoto2022deep,
  author={Matsumoto, Masahiro and Ando, Kazuaki},
  booktitle={2022 IEEE Asia-Pacific Conference on Computer Science and Data Engineering (CSDE)}, 
  title={A Deep Learning Model of Estimating User's Place of Residence Using Tweets and Weather Information}, 
  year={2022},
  volume={},
  number={},
  pages={1-6},
  keywords={Deep learning;Social networking (online);Blogs;Neural networks;Urban areas;Sociology;Earthquakes;Twitter;location estimation;deep learning;weather information},
  doi={10.1109/CSDE56538.2022.10089341}}

@inproceedings{do2018twitter,
  title={Twitter user geolocation using deep multiview learning},
  author={Do, Tien Huu and Nguyen, Duc Minh and Tsiligianni, Evaggelia and Cornelis, Bruno and Deligiannis, Nikos},
  booktitle={2018 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={6304--6308},
  year={2018},
  organization={IEEE}
}

@article{oh2023pre,
  title={Pre-training local and non-local geographical influences with contrastive learning},
  author={Oh, Byungkook and Suh, Ilhyun and Cha, Kihoon and Kim, Junbeom and Park, Goeon and Jeong, Sihyun},
  journal={Knowledge-Based Systems},
  volume={259},
  pages={110016},
  year={2023},
  publisher={Elsevier}
}


@article{fang2023representing,
  title={Representing Spatial Data with Graph Contrastive Learning},
  author={Fang, Lanting and Kou, Ze and Yang, Yulian and Li, Tao},
  journal={Remote Sensing},
  volume={15},
  number={4},
  pages={880},
  year={2023},
  publisher={MDPI}
}
@article{ZOLA2020102312,
title = {A Google Trends spatial clustering approach for a worldwide Twitter user geolocation},
journal = {Information Processing \& Management},
volume = {57},
number = {6},
pages = {102312},
year = {2020},
issn = {0306-4573},
doi = {https://doi.org/10.1016/j.ipm.2020.102312},
url = {https://www.sciencedirect.com/science/article/pii/S0306457320308074},
author = {Paola Zola and Costantino Ragno and Paulo Cortez},
keywords = {City-level geolocation, Clustering, Google Trends, Natural language processing, Twitter},
abstract = {User location data is valuable for diverse social media analytics. In this paper, we address the non-trivial task of estimating a worldwide city-level Twitter user location considering only historical tweets. We propose a purely unsupervised approach that is based on a synthetic geographic sampling of Google Trends (GT) city-level frequencies of tweet nouns and three clustering algorithms. The approach was validated empirically by using a recently collected dataset, with 3,268 worldwide city-level locations of Twitter users, obtaining competitive results when compared with a state-of-the-art Word Distribution (WD) user location estimation method. The best overall results were achieved by the GT noun DBSCAN (GTN-DB) method, which is computationally fast, and correctly predicts the ground truth locations of 15%, 23%, 39% and 58% of the users for tolerance distances of 250 km, 500 km, 1,000 km and 2,000 km.}
}
@inproceedings{huang2021m3g,
  title={M3G: Learning urban neighborhood representation from multi-modal multi-graph},
  author={Huang, Tianyuan and Wang, Zhecheng and Sheng, Hao and Ng, Andrew Y and Rajagopal, Ram},
  booktitle={Proceedings of the DeepSpatial 2021: 2nd ACM KDD Workshop on Deep Learning for Spatio-Temporal Data, Applications and Systems},
  year={2021}
}

@article{bai2023geographic,
  title={Geographic mapping with unsupervised multi-modal representation learning from VHR images and POIs},
  author={Bai, Lubin and Huang, Weiming and Zhang, Xiuyuan and Du, Shihong and Cong, Gao and Wang, Haoyu and Liu, Bo},
  journal={ISPRS Journal of Photogrammetry and Remote Sensing},
  volume={201},
  pages={193--208},
  year={2023},
  publisher={Elsevier}
}

@article{zhou2022metageo,
  title={MetaGeo: a general framework for social user geolocation identification with few-shot learning},
  author={Zhou, Fan and Qi, Xiuxiu and Zhang, Kunpeng and Trajcevski, Goce and Zhong, Ting},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2022},
  publisher={IEEE}
}

@article{suwaileh2022disaster,
  title={When a disaster happens, we are ready: Location mention recognition from crisis tweets},
  author={Suwaileh, Reem and Elsayed, Tamer and Imran, Muhammad and Sajjad, Hassan},
  journal={International Journal of Disaster Risk Reduction},
  volume={78},
  pages={103107},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{tao2021episodic,
  title={An episodic learning based geolocation detection framework for imbalanced data},
  author={Tao, Hemeng and Gao, Yang and Wang, Zhuoyi and Khan, Latifur and Thuraisingham, Bhavani},
  booktitle={2021 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--8},
  year={2021}
}

@InProceedings{thomas2018twitter,
author="Thomas, Philippe
and Hennig, Leonhard",
editor="Rehm, Georg
and Declerck, Thierry",
title="Twitter Geolocation Prediction Using Neural Networks",
booktitle="Language Technologies for the Challenges of the Digital Age",
year="2018",
publisher="Springer International Publishing",
address="Cham",
pages="248--255",
abstract="Knowing the location of a user is important for several use cases, such as location specific recommendations, demographic analysis, or monitoring of disaster outbreaks. We present a bottom up study on the impact of text- and metadata-derived contextual features for Twitter geolocation prediction. The final model incorporates individual types of tweet information and achieves state-of-the-art performance on a publicly available test set. The source code of our implementation, together with pretrained models, is freely available at https://github.com/Erechtheus/geolocation.",
isbn="978-3-319-73706-5"
}

@misc{li2024leveraging,
      title={Leveraging Contrastive Learning for Few-shot Geolocation of Social Posts}, 
      author={Menglin Li and Kwan Hui Lim},
      year={2024},
      eprint={2403.00786},
      archivePrefix={arXiv},
      primaryClass={cs.IR}
}

@article{zheng2018survey,
  title={A survey of location prediction on twitter},
  author={Zheng, Xin and Han, Jialong and Sun, Aixin},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={30},
  number={9},
  pages={1652--1671},
  year={2018},
  publisher={IEEE}
}

@inproceedings{gao-etal-2021-simcse,
    title = "{S}im{CSE}: Simple Contrastive Learning of Sentence Embeddings",
    author = "Gao, Tianyu  and
      Yao, Xingcheng  and
      Chen, Danqi",
    booktitle = "Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing",
    month = nov,
    year = "2021",
    url = "https://aclanthology.org/2021.emnlp-main.552",
    doi = "10.18653/v1/2021.emnlp-main.552",
    pages = "6894--6910",
    abstract = "This paper presents SimCSE, a simple contrastive learning framework that greatly advances the state-of-the-art sentence embeddings. We first describe an unsupervised approach, which takes an input sentence and predicts itself in a contrastive objective, with only standard dropout used as noise. This simple method works surprisingly well, performing on par with previous supervised counterparts. We find that dropout acts as minimal data augmentation and removing it leads to a representation collapse. Then, we propose a supervised approach, which incorporates annotated pairs from natural language inference datasets into our contrastive learning framework, by using {``}entailment{''} pairs as positives and {``}contradiction{''} pairs as hard negatives. We evaluate SimCSE on standard semantic textual similarity (STS) tasks, and our unsupervised and supervised models using BERT base achieve an average of 76.3{\%} and 81.6{\%} Spearman{'}s correlation respectively, a 4.2{\%} and 2.2{\%} improvement compared to previous best results. We also show{---}both theoretically and empirically{---}that contrastive learning objective regularizes pre-trained embeddings{'} anisotropic space to be more uniform, and it better aligns positive pairs when supervised signals are available.",
}

@article{jiang-etal-2020-know,
    title = "How Can We Know What Language Models Know?",
    author = "Jiang, Zhengbao  and
      Xu, Frank F.  and
      Araki, Jun  and
      Neubig, Graham",
    editor = "Johnson, Mark  and
      Roark, Brian  and
      Nenkova, Ani",
    journal = "Transactions of the Association for Computational Linguistics",
    volume = "8",
    year = "2020",
    address = "Cambridge, MA",
    publisher = "MIT Press",
    url = "https://aclanthology.org/2020.tacl-1.28",
    pages = "423--438",
}

@inproceedings{kliman2015location,
  title={Location, location, location: The impact of geolocation on web search personalization},
  author={Kliman-Silver, Chloe and Hannak, Aniko and Lazer, David and Wilson, Christo and Mislove, Alan},
  booktitle={Proceedings of the 2015 internet measurement conference},
  pages={121--127},
  year={2015}
}

@inproceedings{zhang-etal-2022-changes,
    title = "Changes in Tweet Geolocation over Time: A Study with Carmen 2.0",
    author = "Zhang, Jingyu  and
      DeLucia, Alexandra  and
      Dredze, Mark",
    booktitle = "Proceedings of the Eighth Workshop on Noisy User-generated Text (W-NUT 2022)",
    month = oct,
    year = "2022",
    address = "Gyeongju, Republic of Korea",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.wnut-1.1",
    pages = "1--14",
    abstract = "Researchers across disciplines use Twitter geolocation tools to filter data for desired locations. These tools have largely been trained and tested on English tweets, often originating in the United States from almost a decade ago. Despite the importance of these tools for data curation, the impact of tweet language, country of origin, and creation date on tool performance remains largely unknown. We explore these issues with Carmen, a popular tool for Twitter geolocation. To support this study we introduce Carmen 2.0, a major update which includes the incorporation of GeoNames, a gazetteer that provides much broader coverage of locations. We evaluate using two new Twitter datasets, one for multilingual, multiyear geolocation evaluation, and another for usage trends over time. We found that language, country origin, and time does impact geolocation tool performance.",
}

@inproceedings{Ramponi2023GeoLingItAE,
  title={GeoLingIt at EVALITA 2023: Overview of the Geolocation of Linguistic Variation in Italy Task},
  author={Alan Ramponi and Camilla Casula},
  booktitle={International Workshop on Evaluation of Natural Language and Speech Tools for Italian},
  year={2023},
  url={https://api.semanticscholar.org/CorpusID:261529127}
}

@article{liu2023pre,
  title={Pre-train, prompt, and predict: A systematic survey of prompting methods in natural language processing},
  author={Liu, Pengfei and Yuan, Weizhe and Fu, Jinlan and Jiang, Zhengbao and Hayashi, Hiroaki and Neubig, Graham},
  journal={ACM Computing Surveys},
  volume={55},
  number={9},
  pages={1--35},
  year={2023},
  publisher={ACM New York, NY}
}

@inproceedings{han-etal-2016-twitter,
    title = "{T}witter Geolocation Prediction Shared Task of the 2016 Workshop on Noisy User-generated Text",
    author = "Han, Bo  and
      Rahimi, Afshin  and
      Derczynski, Leon  and
      Baldwin, Timothy",
    editor = "Han, Bo  and
      Ritter, Alan  and
      Derczynski, Leon  and
      Xu, Wei  and
      Baldwin, Tim",
    booktitle = "Proceedings of the 2nd Workshop on Noisy User-generated Text ({WNUT})",
    month = dec,
    year = "2016",
    address = "Osaka, Japan",
    publisher = "The COLING 2016 Organizing Committee",
    url = "https://aclanthology.org/W16-3928",
    pages = "213--217",
    abstract = "This paper presents the shared task for English Twitter geolocation prediction in WNUT 2016. We discuss details of task settings, data preparations and participant systems. The derived dataset and performance figures from each system provide baselines for future research in this realm.",
}

@misc{lutsai2023geolocation,
      title={Geolocation Predicting of Tweets Using BERT-Based Models}, 
      author={Kateryna Lutsai and Christoph H. Lampert},
      year={2023},
      eprint={2303.07865},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@article{qiao2023twitter,
  title={Twitter user geolocation based on heterogeneous relationship modeling and representation learning},
  author={Qiao, Yaqiong and Luo, Xiangyang and Ma, Jiangtao and Zhang, Meng and Li, Chenliang},
  journal={Information Sciences},
  volume={647},
  pages={119427},
  year={2023},
  publisher={Elsevier}
}

@article{liu2023ugcc,
  title={UGCC: Social Media User Geolocation via Cyclic Coupling},
  author={Liu, Yimin and Luo, Xiangyang and Tao, Zhiyuan and Zhang, Meng and Du, Shaoyong},
  journal={IEEE Transactions on Big Data},
  year={2023},
  publisher={IEEE}
}

@inproceedings{huang-carley-2019-hierarchical,
    title = "A Hierarchical Location Prediction Neural Network for {T}witter User Geolocation",
    author = "Huang, Binxuan  and
      Carley, Kathleen",
    booktitle = "Proceedings of the 2019 EMNLP-IJCNLP",
    month = nov,
    year = "2019",
    url = "https://aclanthology.org/D19-1480",
    doi = "10.18653/v1/D19-1480",
    pages = "4732--4742",
    abstract = "Accurate estimation of user location is important for many online services. Previous neural network based methods largely ignore the hierarchical structure among locations. In this paper, we propose a hierarchical location prediction neural network for Twitter user geolocation. Our model first predicts the home country for a user, then uses the country result to guide the city-level prediction. In addition, we employ a character-aware word embedding layer to overcome the noisy information in tweets. With the feature fusion layer, our model can accommodate various feature combinations and achieves state-of-the-art results over three commonly used benchmarks under different feature settings. It not only improves the prediction accuracy but also greatly reduces the mean error distance.",
}

@article{luo2022clip4clip,
  title={Clip4clip: An empirical study of clip for end to end video clip retrieval and captioning},
  author={Luo, Huaishao and Ji, Lei and Zhong, Ming and Chen, Yang and Lei, Wen and Duan, Nan and Li, Tianrui},
  journal={Neurocomputing},
  volume={508},
  pages={293--304},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{he2020momentum,
  title={Momentum contrast for unsupervised visual representation learning},
  author={He, Kaiming and Fan, Haoqi and Wu, Yuxin and Xie, Saining and Girshick, Ross},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={9729--9738},
  year={2020}
}

@article{khosla2020supervised,
  title={Supervised contrastive learning},
  author={Khosla, Prannay and Teterwak, Piotr and Wang, Chen and Sarna, Aaron and Tian, Yonglong and Isola, Phillip and Maschinot, Aaron and Liu, Ce and Krishnan, Dilip},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={18661--18673},
  year={2020}
}

@inproceedings{zhang2022pointclip,
  title={Pointclip: Point cloud understanding by clip},
  author={Zhang, Renrui and Guo, Ziyu and Zhang, Wei and Li, Kunchang and Miao, Xupeng and Cui, Bin and Qiao, Yu and Gao, Peng and Li, Hongsheng},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8552--8562},
  year={2022}
}

@inproceedings{zhong2021factual,
  title={Factual Probing Is $[MASK]$: Learning vs. Learning to Recall},
  author={Zhong, Zexuan and Friedman, Dan and Chen, Danqi},
  booktitle={Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
  pages={5017--5033},
  year={2021}
}

@inproceedings{shin2020autoprompt,
  title={AutoPrompt: Eliciting Knowledge from Language Models with Automatically Generated Prompts},
  author={Shin, Taylor and Razeghi, Yasaman and Logan IV, Robert L and Wallace, Eric and Singh, Sameer},
  booktitle={Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
  pages={4222--4235},
  year={2020}
}

@inproceedings{radford2021learning,
  title={Learning transferable visual models from natural language supervision},
  author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and others},
  booktitle={International conference on machine learning},
  pages={8748--8763},
  year={2021}
}

@article{li2021align,
  title={Align before fuse: Vision and language representation learning with momentum distillation},
  author={Li, Junnan and Selvaraju, Ramprasaath and Gotmare, Akhilesh and Joty, Shafiq and Xiong, Caiming and Hoi, Steven Chu Hong},
  journal={Advances in neural information processing systems},
  volume={34},
  pages={9694--9705},
  year={2021}
}

@inproceedings{chen2020simple,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1597--1607},
  year={2020}
}

@article{vinker2022clipasso,
  title={Clipasso: Semantically-aware object sketching},
  author={Vinker, Yael and Pajouheshgar, Ehsan and Bo, Jessica Y and Bachmann, Roman Christian and Bermano, Amit Haim and Cohen-Or, Daniel and Zamir, Amir and Shamir, Ariel},
  journal={ACM Transactions on Graphics (TOG)},
  volume={41},
  number={4},
  pages={1--11},
  year={2022},
  publisher={ACM New York, NY, USA}
}

@article{wang2021actionclip,
  title={Actionclip: A new paradigm for video action recognition},
  author={Wang, Mengmeng and Xing, Jiazheng and Liu, Yong},
  journal={arXiv preprint arXiv:2109.08472},
  year={2021}
}



@inproceedings{poulston2017hyperlocal,
  title={Hyperlocal home location identification of twitter profiles},
  author={Poulston, Adam and Stevenson, Mark and Bontcheva, Kalina},
  booktitle={Proceedings of the 28th ACM conference on hypertext and social media},
  pages={45--54},
  year={2017}
}

@inproceedings{kavak2018fine,
  title={Fine-scale prediction of people’s home location using social media footprints},
  author={Kavak, Hamdi and Vernon-Bido, Daniele and Padilla, Jose J},
  booktitle={International Conference on Social Computing, Behavioral-Cultural Modeling and Prediction and Behavior Representation in Modeling and Simulation},
  pages={183--189},
  year={2018}
}

@inproceedings{mcgee2013location,
  title={Location prediction in social media based on tie strength},
  author={McGee, Jeffrey and Caverlee, James and Cheng, Zhiyuan},
  booktitle={Proceedings of the 22nd ACM international conference on Information \& Knowledge Management},
  pages={459--468},
  year={2013}
}

@inproceedings{wagenseller2019location,
  title={Location Prediction with Communities in User Ego-Net in Social Media},
  author={Wagenseller, Paul and Avram, Adrian and Jiang, Eric and Wang, Feng and Zhao, Yunpeng},
  booktitle={ICC 2019-2019 IEEE International Conference on Communications (ICC)},
  pages={1--6},
  year={2019}
}

@inproceedings{jurgens2015geolocation,
  title={Geolocation prediction in twitter using social networks: A critical analysis and review of current practice},
  author={Jurgens, David and Finethy, Tyler and McCorriston, James and Xu, Yi and Ruths, Derek},
  booktitle={Proceedings of the International AAAI Conference on Web and Social Media},
  volume={9},
  number={1},
  year={2015}
}

@article{rahimi2015twitter,
  title={Twitter user geolocation using a unified text and network prediction model},
  author={Rahimi, Afshin and Cohn, Trevor and Baldwin, Timothy},
  journal={arXiv preprint arXiv:1506.08259},
  year={2015}
}

@article{rodrigues2016exploring,
  title={Exploring multiple evidence to infer users’ location in Twitter},
  author={Rodrigues, Erica and Assun{\c{c}}{\~a}o, Renato and Pappa, Gisele L and Renno, Diogo and Meira Jr, Wagner},
  journal={Neurocomputing},
  volume={171},
  pages={30--38},
  year={2016},
  publisher={Elsevier}
}

@inproceedings{xu2014location,
  title={Location prediction in social media based on contents and graphs},
  author={Xu, Dan and Yang, Shiqiang},
  booktitle={2014 Fourth International Conference on Communication Systems and Network Technologies},
  pages={1177--1181},
  year={2014}
}

@inproceedings{xu2014find,
  title={Find you from your friends: Graph-based residence location prediction for users in social media},
  author={Xu, Dan and Cui, Peng and Zhu, Wenwu and Yang, Shiqiang},
  booktitle={2014 IEEE international conference on multimedia and expo (ICME)},
  pages={1--6},
  year={2014}
}

@inproceedings{backstrom2010find,
  title={Find me if you can: improving geographical prediction with social and spatial proximity},
  author={Backstrom, Lars and Sun, Eric and Marlow, Cameron},
  booktitle={Proceedings of the 19th international conference on World wide web},
  pages={61--70},
  year={2010}
}

@article{iso2017density,
  publtype={informal},
  author={Hayate Iso and Shoko Wakamiya and Eiji Aramaki},
  title={Density Estimation for Geolocation via Convolutional Mixture Density Network},
  year={2017},
  cdate={1483228800000},
  journal={CoRR},
  volume={abs/1705.02750},
  url={http://arxiv.org/abs/1705.02750}
}

@inproceedings{liu2021crisisbert,
  title={CrisisBERT: a Robust Transformer for Crisis Classification and Contextual Crisis Embedding},
  author={Liu, Junhua and Singhal, Trisha and Blessing, Lucienne T.M. and Wood, Kristin L. and Lim, Kwan Hui},
  booktitle={Proceedings of the 32nd ACM Conference on Hypertext and Social Media},
  pages={133--141},
  year={2021}
}

@inproceedings{liu2020strategic,
  title={Strategic and Crowd-aware Itinerary Recommendation},
  author={Liu, Junhua and Wood, Kristin L and Lim, Kwan Hui},
  booktitle={Proceedings of the 2020 European Conference on Machine Learning and Knowledge Discovery in Databases (ECML-PKDD'20)},
  year={2020}
}

@inproceedings{rahimi2017continuous,
    title = "Continuous Representation of Location for Geolocation and Lexical Dialectology using Mixture Density Networks",
    author = "Rahimi, Afshin  and
      Baldwin, Timothy  and
      Cohn, Trevor",
    booktitle = "Proceedings of the 2017 Conference on Empirical Methods in Natural Language Processing",
    month = sep,
    year = "2017",
    url = "https://aclanthology.org/D17-1016",
    doi = "10.18653/v1/D17-1016",
    pages = "167--176",
    abstract = "We propose a method for embedding two-dimensional locations in a continuous vector space using a neural network-based model incorporating mixtures of Gaussian distributions, presenting two model variants for text-based geolocation and lexical dialectology. Evaluated over Twitter data, the proposed model outperforms conventional regression-based geolocation and provides a better estimate of uncertainty. We also show the effectiveness of the representation for predicting words from location in lexical dialectology, and evaluate it using the DARE dataset.",
}

@inproceedings{2018arXiv180205365P,
    title = "Deep Contextualized Word Representations",
    author = "Peters, Matthew E.  and
      Neumann, Mark  and
      Iyyer, Mohit  and
      Gardner, Matt  and
      Clark, Christopher  and
      Lee, Kenton  and
      Zettlemoyer, Luke",
    booktitle = "Proceedings of the 2018 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long Papers)",
    month = jun,
    year = "2018",
    url = "https://aclanthology.org/N18-1202",
    doi = "10.18653/v1/N18-1202",
    pages = "2227--2237",
    abstract = "We introduce a new type of deep contextualized word representation that models both (1) complex characteristics of word use (e.g., syntax and semantics), and (2) how these uses vary across linguistic contexts (i.e., to model polysemy). Our word vectors are learned functions of the internal states of a deep bidirectional language model (biLM), which is pre-trained on a large text corpus. We show that these representations can be easily added to existing models and significantly improve the state of the art across six challenging NLP problems, including question answering, textual entailment and sentiment analysis. We also present an analysis showing that exposing the deep internals of the pre-trained network is crucial, allowing downstream models to mix different types of semi-supervision signals.",
}

@inproceedings{devlin2018bert,
    title = "{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding",
    author = "Devlin, Jacob  and
      Chang, Ming-Wei  and
      Lee, Kenton  and
      Toutanova, Kristina",
    booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)",
    month = jun,
    year = "2019",
    url = "https://aclanthology.org/N19-1423",
    doi = "10.18653/v1/N19-1423",
    pages = "4171--4186",
    abstract = "We introduce a new language representation model called BERT, which stands for Bidirectional Encoder Representations from Transformers. Unlike recent language representation models (Peters et al., 2018a; Radford et al., 2018), BERT is designed to pre-train deep bidirectional representations from unlabeled text by jointly conditioning on both left and right context in all layers. As a result, the pre-trained BERT model can be fine-tuned with just one additional output layer to create state-of-the-art models for a wide range of tasks, such as question answering and language inference, without substantial task-specific architecture modifications. BERT is conceptually simple and empirically powerful. It obtains new state-of-the-art results on eleven natural language processing tasks, including pushing the GLUE score to 80.5 (7.7 point absolute improvement), MultiNLI accuracy to 86.7{\%} (4.6{\%} absolute improvement), SQuAD v1.1 question answering Test F1 to 93.2 (1.5 point absolute improvement) and SQuAD v2.0 Test F1 to 83.1 (5.1 point absolute improvement).",
}

@inproceedings{miura2017unifying,
  title={Unifying text, metadata, and user network representations with a neural network for geolocation prediction},
  author={Miura, Yasuhide and Taniguchi, Motoki and Taniguchi, Tomoki and Ohkuma, Tomoko},
  booktitle={Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={1260--1272},
  year={2017}
}

@inproceedings{wing2014hierarchical,
  title={Hierarchical discriminative classification for text-based geolocation},
  author={Wing, Benjamin and Baldridge, Jason},
  booktitle={Proceedings of the 2014 conference on empirical methods in natural language processing (EMNLP)},
  pages={336--348},
  year={2014}
}

@inproceedings{fei2019location,
  title={Location Prediction for Social Media Users Based on Information Fusion},
  author={Fei, Gaolei and Liu, Yang and Cheng, Yong and Yu, Fucai and Hu, Guangmin},
  booktitle={International Conference on Algorithms and Architectures for Parallel Processing},
  pages={599--612},
  year={2019}
}

@inproceedings{miura2016simple,
  title={A simple scalable neural networks based model for geolocation prediction in twitter},
  author={Miura, Yasuhide and Taniguchi, Motoki and Taniguchi, Tomoki and Ohkuma, Tomoko},
  booktitle={Proceedings of the 2nd Workshop on Noisy User-generated Text (WNUT)},
  pages={235--239},
  year={2016}
}

@misc{internet2016twitter,
  title={Twitter usage statistics},
  author={Internet Live Stats},
  year={2016},
  publisher={InternetLiveStats. com}
}#25

@article{han2020extracting,
  title={Extracting representative images of tourist attractions from Flickr by combing an improved cluster method and multiple deep learning models},
  author={Han, Shanshan and Ren, Fu and Du, Qingyun and Gui, Dawei},
  journal={ISPRS International Journal of Geo-Information},
  volume={9},
  number={2},
  pages={81},
  year={2020},
  publisher={Multidisciplinary Digital Publishing Institute}
}#26

@article{gruzd2011imagining,
  title={Imagining Twitter as an imagined community},
  author={Gruzd, Anatoliy and Wellman, Barry and Takhteyev, Yuri},
  journal={American Behavioral Scientist},
  volume={55},
  number={10},
  pages={1294--1318},
  year={2011},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@inproceedings{cameron2012emergency,
  title={Emergency situation awareness from twitter for crisis management},
  author={Cameron, Mark A and Power, Robert and Robinson, Bella and Yin, Jie},
  booktitle={Proceedings of the 21st international conference on world wide web},
  pages={695--698},
  year={2012}
}#27

@article{imran2015processing,
  title={Processing social media messages in mass emergency: A survey},
  author={Imran, Muhammad and Castillo, Carlos and Diaz, Fernando and Vieweg, Sarah},
  journal={ACM Computing Surveys (CSUR)},
  volume={47},
  number={4},
  pages={1--38},
  year={2015},
  publisher={ACM New York, NY, USA}
}#28

@article{middleton2013real,
  title={Real-time crisis mapping of natural disasters using social media},
  author={Middleton, Stuart E and Middleton, Lee and Modafferi, Stefano},
  journal={IEEE Intelligent Systems},
  volume={29},
  number={2},
  pages={9--17},
  year={2013},
  publisher={IEEE}
}#29

@inproceedings{sakaki2010earthquake,
  title={Earthquake shakes twitter users: real-time event detection by social sensors},
  author={Sakaki, Takeshi and Okazaki, Makoto and Matsuo, Yutaka},
  booktitle={Proceedings of the 19th international conference on World wide web},
  pages={851--860},
  year={2010}
}#30

@inproceedings{brown2012importance,
  title={The importance of being placefriends: discovering location-focused online communities},
  author={Brown, Chlo{\"e} and Nicosia, Vincenzo and Scellato, Salvatore and Noulas, Anastasios and Mascolo, Cecilia},
  booktitle={Proceedings of the 2012 ACM workshop on Workshop on online social networks},
  pages={31--36},
  year={2012}
}#31

@article{crandall2010inferring,
  title={Inferring social ties from geographic coincidences},
  author={Crandall, David J and Backstrom, Lars and Cosley, Dan and Suri, Siddharth and Huttenlocher, Daniel and Kleinberg, Jon},
  journal={Proceedings of the National Academy of Sciences},
  volume={107},
  number={52},
  pages={22436--22441},
  year={2010},
  publisher={National Acad Sciences}
}#32

@inproceedings{lim2015detecting,
  title={Detecting location-centric communities using social-spatial links with temporal constraints},
  author={Lim, Kwan Hui and Chan, Jeffrey and Leckie, Christopher and Karunasekera, Shanika},
  booktitle={European Conference on information retrieval},
  pages={489--494},
  year={2015}
}#33

@article{wang2021semantic,
  title={Semantic Place Prediction With User Attribute in Social Media},
  author={Wang, Ning and Liu, Boqian and Niu, Muyao and Meng, Kaidi and Li, Haojie and Liu, Bin and Wang, Zhihui},
  journal={IEEE MultiMedia},
  volume={28},
  number={4},
  pages={29--37},
  year={2021},
  publisher={IEEE}
}

@inproceedings{zhou2020hierarchy,
  title={Hierarchy-aware global model for hierarchical text classification},
  author={Zhou, Jie and Ma, Chunping and Long, Dingkun and Xu, Guangwei and Ding, Ning and Zhang, Haoyu and Xie, Pengjun and Liu, Gongshen},
  booktitle={Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
  pages={1106--1117},
  year={2020}
}

@inproceedings{kowsari2017hdltex,
  title={Hdltex: Hierarchical deep learning for text classification},
  author={Kowsari, Kamran and Brown, Donald E and Heidarysafa, Mojtaba and Meimandi, Kiana Jafari and Gerber, Matthew S and Barnes, Laura E},
  booktitle={2017 16th IEEE international conference on machine learning and applications (ICMLA)},
  pages={364--371},
  year={2017}
}

@inproceedings{huang12019hierarchical,
  title={Hierarchical multi-label text classification: An attention-based recurrent network approach},
  author={Huang, Wei and Chen, Enhong and Liu, Qi and Chen, Yuying and Huang, Zai and Liu, Yang and Zhao, Zhou and Zhang, Dan and Wang, Shijin},
  booktitle={Proceedings of the 28th ACM international conference on information and knowledge management},
  pages={1051--1060},
  year={2019}
}

@inproceedings{Johnson2015EffectiveUO,
  title={Effective Use of Word Order for Text Categorization with Convolutional Neural Networks},
  author={Rie Johnson and Tong Zhang},
  booktitle={NAACL},
  year={2015}
}

@article{radford2018improving,
  title={Improving language understanding by generative pre-training},
  author={Radford, Alec and Narasimhan, Karthik and Salimans, Tim and Sutskever, Ilya and others},
  year={2018},
  publisher={OpenAI}
}

@inproceedings{taylor2018travel,
  title={Travel itinerary recommendations with must-see points-of-interest},
  author={Taylor, Kendall and Lim, Kwan Hui and Chan, Jeffrey},
  booktitle={Companion Proceedings of the The Web Conference 2018},
  pages={1198--1205},
  year={2018}
}

@inproceedings{zhou2021informer,
  title={Informer: Beyond efficient transformer for long sequence time-series forecasting},
  author={Zhou, Haoyi and Zhang, Shanghang and Peng, Jieqi and Zhang, Shuai and Li, Jianxin and Xiong, Hui and Zhang, Wancai},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  pages={11106--11115},
  year={2021}
}

@article{ruder2017overview,
  title={An overview of multi-task learning in deep neural networks},
  author={Ruder, Sebastian},
  journal={arXiv preprint arXiv:1706.05098},
  year={2017}
}

@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{huang2019hierarchical,
    title = "A Hierarchical Location Prediction Neural Network for {T}witter User Geolocation",
    author = "Huang, Binxuan  and
      Carley, Kathleen",
    booktitle = "Proceedings of the 2019 EMNLP-IJCNLP",
    month = nov,
    year = "2019",
    url = "https://aclanthology.org/D19-1480",
    doi = "10.18653/v1/D19-1480",
    pages = "4732--4742",
    abstract = "Accurate estimation of user location is important for many online services. Previous neural network based methods largely ignore the hierarchical structure among locations. In this paper, we propose a hierarchical location prediction neural network for Twitter user geolocation. Our model first predicts the home country for a user, then uses the country result to guide the city-level prediction. In addition, we employ a character-aware word embedding layer to overcome the noisy information in tweets. With the feature fusion layer, our model can accommodate various feature combinations and achieves state-of-the-art results over three commonly used benchmarks under different feature settings. It not only improves the prediction accuracy but also greatly reduces the mean error distance.",
}


@article{silla2011survey,
  title={A survey of hierarchical classification across different application domains},
  author={Silla, Carlos N and Freitas, Alex A},
  journal={Data Mining and Knowledge Discovery},
  volume={22},
  number={1},
  pages={31--72},
  year={2011},
  publisher={Springer}
}

@inproceedings{zhong2020interpreting,
  title={Interpreting Twitter user geolocation},
  author={Zhong, Ting and Wang, Tianliang and Zhou, Fan and Trajcevski, Goce and Zhang, Kunpeng and Yang, Yi},
  booktitle={Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
  pages={853--859},
  year={2020}
}

@inproceedings{cheng2010you,
  title={You are where you tweet: a content-based approach to geo-locating twitter users},
  author={Cheng, Zhiyuan and Caverlee, James and Lee, Kyumin},
  booktitle={Proceedings of the 19th ACM international conference on Information and knowledge management},
  pages={759--768},
  year={2010}
}

@inproceedings{meng2019weakly,
  title={Weakly-supervised hierarchical text classification},
  author={Meng, Yu and Shen, Jiaming and Zhang, Chao and Han, Jiawei},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={33},
  pages={6826--6833},
  year={2019}
}

@inproceedings{kordopatis2015geotagging,
  title={Geotagging social media content with a refined language modelling approach},
  author={Kordopatis-Zilos, Giorgos and Papadopoulos, Symeon and Kompatsiaris, Yiannis},
  booktitle={Pacific-Asia Workshop on Intelligence and Security Informatics},
  pages={21--40},
  year={2015}
}

@article{li2018location,
  title={Location inference for non-geotagged tweets in user timelines},
  author={Li, Pengfei and Lu, Hua and Kanhabua, Nattiya and Zhao, Sha and Pan, Gang},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={31},
  number={6},
  pages={1150--1165},
  year={2018},
  publisher={IEEE}
}


@inproceedings{tigunova2015location,
  title={Location prediction via social contents and behaviors: location-aware behavioral LDA},
  author={Tigunova, Anna and Lee, JooYoung and Nobari, Sadegh},
  booktitle={2015 IEEE International Conference on Data Mining Workshop (ICDMW)},
  pages={1131--1135},
  year={2015}
}

@article{singh2019event,
  title={Event classification and location prediction from tweets during disasters},
  author={Singh, Jyoti Prakash and Dwivedi, Yogesh K and Rana, Nripendra P and Kumar, Abhinav and Kapoor, Kawaljeet Kaur},
  journal={Annals of Operations Research},
  volume={283},
  number={1},
  pages={737--757},
  year={2019},
  publisher={Springer}
}

@article{kulkarni2020spatial,
  title={Spatial language representation with multi-level geocoding},
  author={Kulkarni, Sayali and Jain, Shailee and Hosseini, Mohammad Javad and Baldridge, Jason and Ie, Eugene and Zhang, Li},
  journal={arXiv preprint arXiv:2008.09236},
  year={2020}
}

@inproceedings{scherrer2021social,
  title={Social media variety geolocation with geobert},
  author={Scherrer, Yves and Ljube{\v{s}}i{\'c}, Nikola},
  booktitle={Proceedings of the Eighth Workshop on NLP for Similar Languages, Varieties and Dialects},
  year={2021}
}

@inproceedings{mircea2020real,
  title={Real-time classification, geolocation and interactive visualization of COVID-19 information shared on social media to better understand global developments},
  author={Mircea, Andrei},
  booktitle={Proceedings of the 1st Workshop on NLP for COVID-19 (Part 2) at EMNLP 2020},
  year={2020}
}

@inproceedings{kordopatis2016placing,
  title={Placing Images with Refined Language Models and Similarity Search with PCA-reduced VGG Features.},
  author={Kordopatis-Zilos, Giorgos and Popescu, Adrian and Papadopoulos, Symeon and Kompatsiaris, Yiannis},
  booktitle={MediaEval},
  year={2016}
}

@article{middleton2018location,
  title={Location extraction from social media: Geoparsing, location disambiguation, and geotagging},
  author={Middleton, Stuart E and Kordopatis-Zilos, Giorgos and Papadopoulos, Symeon and Kompatsiaris, Yiannis},
  journal={ACM Transactions on Information Systems (TOIS)},
  volume={36},
  number={4},
  pages={1--27},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@article{zhong2020multiple,
  title={Multiple-aspect attentional graph neural networks for online social network user localization},
  author={Zhong, Ting and Wang, Tianliang and Wang, Jiahao and Wu, Jin and Zhou, Fan},
  journal={IEEE Access},
  volume={8},
  pages={95223--95234},
  year={2020},
  publisher={IEEE}
}

@inproceedings{sadilek2012finding,
  title={Finding your friends and following them to where you are},
  author={Sadilek, Adam and Kautz, Henry and Bigham, Jeffrey P},
  booktitle={Proceedings of the fifth ACM international conference on Web search and data mining},
  pages={723--732},
  year={2012}
}#34

@article{sloan2013knowing,
  title={Knowing the tweeters: Deriving sociologically relevant demographics from Twitter},
  author={Sloan, Luke and Morgan, Jeffrey and Housley, William and Williams, Matthew and Edwards, Adam and Burnap, Pete and Rana, Omer},
  journal={Sociological research online},
  volume={18},
  number={3},
  pages={74--84},
  year={2013},
  publisher={SAGE Publications Sage UK: London, England}
}#35

@article{zielstra2013positional,
  title={Positional accuracy analysis of Flickr and Panoramio images for selected world regions},
  author={Zielstra, Dennis and Hochmair, Hartwig H},
  journal={Journal of Spatial Science},
  volume={58},
  number={2},
  pages={251--273},
  year={2013},
  publisher={Taylor \& Francis}
}#36

@inproceedings{ouaret2019random,
  title={Random Forest location prediction from social networks during disaster events},
  author={Ouaret, Rachid and Birregah, Babiga and Soulier, Eddie and Auclair, Samuel and Boulahya, Faiza},
  booktitle={2019 Sixth International Conference on Social Networks Analysis, Management and Security (SNAMS)},
  pages={535--540},
  year={2019}
}

@article{ozdikis2019locality,
  title={Locality-adapted kernel densities of term co-occurrences for location prediction of tweets},
  author={Ozdikis, Ozer and Ramampiaro, Heri and N{\o}rv{\aa}g, Kjetil},
  journal={Information Processing \& Management},
  volume={56},
  number={4},
  pages={1280--1299},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{han2012geolocation,
  title={Geolocation prediction in social media data by finding location indicative words},
  author={Han, Bo and Cook, Paul and Baldwin, Timothy},
  booktitle={Proceedings of COLING 2012},
  pages={1045--1062},
  year={2012}
}

@inproceedings{grace2019expanding,
  title={Expanding Awareness: Comparing Location, Keyword, and Network Filtering Methods to Collect Hyperlocal Social Media Data},
  author={Grace, Rob and Halse, Shane and Aurite, William and Montarnal, Aur{\'e}lie and Tapia, Andrea},
  booktitle={Proceedings of the 52nd Hawaii International Conference on System Sciences},
  year={2019}
}

@article{mazumdar2018hidden,
  title={Hidden location prediction using check-in patterns in location-based social networks},
  author={Mazumdar, Pramit and Patra, Bidyut Kr and Babu, Korra Sathya and Lock, Russell},
  journal={Knowledge and Information Systems},
  volume={57},
  number={3},
  pages={571--601},
  year={2018},
  publisher={Springer}
}

@inproceedings{chong2017exploiting,
  title={Exploiting contextual information for fine-grained tweet geolocation},
  author={Chong, Wen-Haw and Lim, Ee-Peng},
  booktitle={Proceedings of the International AAAI Conference on Web and Social Media},
  volume={11},
  year={2017}
}

@inproceedings{pliakos2014simultaneous,
  title={Simultaneous image tagging and geo-location prediction within hypergraph ranking framework},
  author={Pliakos, Konstantinos and Kotropoulos, Constantine},
  booktitle={2014 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={6894--6898},
  year={2014}
}

@inproceedings{cha2015twitter,
  title={Twitter geolocation and regional classification via sparse coding},
  author={Cha, Miriam and Gwon, Youngjune and Kung, HT},
  booktitle={Ninth International AAAI Conference on Web and Social Media},
  year={2015}
}

@inproceedings{liu2018location,
  title={Location prediction in social networks},
  author={Liu, Rong and Cong, Guanglin and Zheng, Bolong and Zheng, Kai and Su, Han},
  booktitle={Asia-Pacific Web (APWeb) and Web-Age Information Management (WAIM) Joint International Conference on Web and Big Data},
  pages={151--165},
  year={2018}
}

@article{qian2017probabilistic,
  title={A probabilistic framework for location inference from social media},
  author={Qian, Yujie and Tang, Jie and Yang, Zhilin and Huang, Binxuan and Wei, Wei and Carley, Kathleen M},
  journal={arXiv preprint arXiv:1702.07281},
  year={2017}
}

@article{mousset2020end,
  title={End-to-End Neural Matching for Semantic Location Prediction of Tweets},
  author={Mousset, Paul and Pitarch, Yoann and Tamine, Lynda},
  journal={ACM Transactions on Information Systems (TOIS)},
  volume={39},
  number={1},
  pages={1--35},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@article{chong2018exploiting,
  title={Exploiting user and venue characteristics for fine-grained tweet geolocation},
  author={Chong, Wen-Haw and Lim, Ee-Peng},
  journal={ACM Transactions on Information Systems (TOIS)},
  volume={36},
  number={3},
  pages={1--34},
  year={2018},
  publisher={ACM New York, NY, USA}
} #7

@inproceedings{chi2016geolocation,
  title={Geolocation prediction in twitter using location indicative words and textual features},
  author={Chi, Lianhua and Lim, Kwan Hui and Alam, Nebula and Butler, Christopher J},
  booktitle={Proceedings of the 2nd Workshop on Noisy User-generated Text (WNUT)},
  pages={227--234},
  year={2016}
}#6

@article{zohar2021geolocating,
  title={Geolocating tweets via spatial inspection of information inferred from tweet meta-fields},
  author={Zohar, Motti},
  journal={International Journal of Applied Earth Observation and Geoinformation},
  volume={105},
  pages={102593},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{mahmud2012tweet,
  title={Where is this tweet from? inferring home locations of twitter users},
  author={Mahmud, Jalal and Nichols, Jeffrey and Drews, Clemens},
  booktitle={Proceedings of the International AAAI Conference on Web and Social Media},
  volume={6},
  year={2012}
}# 19

@article{han2014text,
  title={Text-based twitter user geolocation prediction},
  author={Han, Bo and Cook, Paul and Baldwin, Timothy},
  journal={Journal of Artificial Intelligence Research},
  volume={49},
  pages={451--500},
  year={2014}
}

@inproceedings{ozdikis2018spatial,
  title={Spatial statistics of term co-occurrences for location prediction of tweets},
  author={Ozdikis, Ozer and Ramampiaro, Heri and N{\o}rv{\aa}g, Kjetil},
  booktitle={European Conference on Information Retrieval},
  pages={494--506},
  year={2018}
}

@inproceedings{lourentzou2017text,
  title={Text-based geolocation prediction of social media users with neural networks},
  author={Lourentzou, Ismini and Morales, Alex and Zhai, ChengXiang},
  booktitle={2017 IEEE International Conference on Big Data (Big Data)},
  pages={696--705},
  year={2017}
}

@inproceedings{huang2017predicting,
  title={On predicting geolocation of tweets using convolutional neural networks},
  author={Huang, Binxuan and Carley, Kathleen M},
  booktitle={International conference on social computing, behavioral-cultural modeling and prediction and behavior representation in modeling and simulation},
  pages={281--291},
  year={2017}
}

@inproceedings{kim-2014-convolutional,
    title = "Convolutional Neural Networks for Sentence Classification",
    author = "Kim, Yoon",
    booktitle = "Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing ({EMNLP})",
    month = oct,
    year = "2014",
    url = "https://www.aclweb.org/anthology/D14-1181",
    doi = "10.3115/v1/D14-1181",
    pages = "1746--1751",
}

@inproceedings{pennington2014glove,
  title={Glove: Global vectors for word representation},
  author={Pennington, Jeffrey and Socher, Richard and Manning, Christopher D},
  booktitle={Proceedings of the 2014 conference on empirical methods in natural language processing (EMNLP)},
  pages={1532--1543},
  year={2014}
}

@inproceedings{rahimi-etal-2017-neural,
    title = "A Neural Model for User Geolocation and Lexical Dialectology",
    author = "Rahimi, Afshin  and
      Cohn, Trevor  and
      Baldwin, Timothy",
    booktitle = "Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)",
    month = jul,
    year = "2017",
    url = "https://www.aclweb.org/anthology/P17-2033",
    doi = "10.18653/v1/P17-2033",
    pages = "209--216",
    abstract = "We propose a simple yet effective text-based user geolocation model based on a neural network with one hidden layer, which achieves state of the art performance over three Twitter benchmark geolocation datasets, in addition to producing word and phrase embeddings in the hidden layer that we show to be useful for detecting dialectal terms. As part of our analysis of dialectal terms, we release DAREDS, a dataset for evaluating dialect term detection methods.",
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@inproceedings{lim2019geotagging,
  title={Geotagging tweets to landmarks using convolutional neural networks with text and posting time},
  author={Lim, Kwan Hui and Karunasekera, Shanika and Harwood, Aaron and George, Yasmeen},
  booktitle={Proceedings of the 24th International Conference on Intelligent User Interfaces: Companion},
  pages={61--62},
  year={2019}
}

@INPROCEEDINGS{ho2022poibert,
  title={POIBERT: A Transformer-based Model for the Tour Recommendation Problem},
  author={Ho, Ngai Lam and Lim, Kwan Hui},
  BOOKTITLE={Proceedings of the 2022 IEEE International Conference on Big Data},
  year={2022}
}

@INPROCEEDINGS{li2022geotagging,
  title={Geotagging Social Media Posts to Landmarks Using Hierarchical BERT (Student Abstract)},
  author={Li, Menglin and Lim, Kwan Hui},
  BOOKTITLE = {Proceedings of the Thirty-Sixth AAAI Conference on Artificial Intelligence (AAAI'22)},
  year={2022}
}

@article{huang2018location,
  title={Location based services: ongoing evolution and research agenda},
  author={Huang, Haosheng and Gartner, Georg and Krisp, Jukka M and Raubal, Martin and Van de Weghe, Nico},
  journal={Journal of Location Based Services},
  volume={12},
  number={2},
  pages={63--93},
  year={2018},
  publisher={Taylor \& Francis}
}

@inproceedings{evans2012intelligent,
  title={An intelligent mobile advertising system (iMAS): Location-based advertising to individuals and business},
  author={Evans, Cain and Moore, Philip and Thomas, Andrew},
  booktitle={2012 Sixth International Conference on Complex, Intelligent, and Software Intensive Systems},
  pages={959--964},
  year={2012}
}

@article{thomee2016yfcc100m,
  title={YFCC100M: The new data in multimedia research},
  author={Thomee, Bart and Shamma, David A and Friedland, Gerald and Elizalde, Benjamin and Ni, Karl and Poland, Douglas and Borth, Damian and Li, Li-Jia},
  journal={Communications of the ACM},
  volume={59},
  number={2},
  pages={64--73},
  year={2016},
  publisher={ACM New York, NY, USA}
}

@inproceedings{li2023transformer,
  title={A transformer-based framework for poi-level social post geolocation},
  author={Li, Menglin and Lim, Kwan Hui and Guo, Teng and Liu, Junhua},
  booktitle={European Conference on Information Retrieval},
  pages={588--604},
  year={2023}
}

@article{li2021disparate,
  title={Disparate patterns of movements and visits to points of interest located in urban hotspots across US metropolitan cities during COVID-19},
  author={Li, Qingchun and Bessell, Liam and Xiao, Xin and Fan, Chao and Gao, Xinyu and Mostafavi, Ali},
  journal={Royal Society open science},
  volume={8},
  number={1},
  pages={201209},
  year={2021},
  publisher={The Royal Society}
}

@article{scalia2022cime,
  title={CIME: Context-aware geolocation of emergency-related posts},
  author={Scalia, Gabriele and Francalanci, Chiara and Pernici, Barbara},
  journal={GeoInformatica},
  volume={26},
  number={1},
  pages={125--157},
  year={2022},
  publisher={Springer}
}

@inproceedings{yan-etal-2021-consert,
    title = "{C}on{SERT}: A Contrastive Framework for Self-Supervised Sentence Representation Transfer",
    author = "Yan, Yuanmeng  and
      Li, Rumei  and
      Wang, Sirui  and
      Zhang, Fuzheng  and
      Wu, Wei  and
      Xu, Weiran",
    booktitle = "Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing",
    month = aug,
    year = "2021",
    url = "https://aclanthology.org/2021.acl-long.393",
    doi = "10.18653/v1/2021.acl-long.393",
    pages = "5065--5075",
    abstract = "Learning high-quality sentence representations benefits a wide range of natural language processing tasks. Though BERT-based pre-trained language models achieve high performance on many downstream tasks, the native derived sentence representations are proved to be collapsed and thus produce a poor performance on the semantic textual similarity (STS) tasks. In this paper, we present ConSERT, a Contrastive Framework for Self-Supervised SEntence Representation Transfer, that adopts contrastive learning to fine-tune BERT in an unsupervised and effective way. By making use of unlabeled texts, ConSERT solves the collapse issue of BERT-derived sentence representations and make them more applicable for downstream tasks. Experiments on STS datasets demonstrate that ConSERT achieves an 8{\%} relative improvement over the previous state-of-the-art, even comparable to the supervised SBERT-NLI. And when further incorporating NLI supervision, we achieve new state-of-the-art performance on STS tasks. Moreover, ConSERT obtains comparable results with only 1000 samples available, showing its robustness in data scarcity scenarios.",
}

@inproceedings{
wang2022simvlm,
title={Sim{VLM}: Simple Visual Language Model Pretraining with Weak Supervision},
author={Zirui Wang and Jiahui Yu and Adams Wei Yu and Zihang Dai and Yulia Tsvetkov and Yuan Cao},
booktitle={International Conference on Learning Representations},
year={2022},
url={https://openreview.net/forum?id=GUrhfTuf_3}
}

@inproceedings{houlsby2019parameter,
  title={Parameter-efficient transfer learning for NLP},
  author={Houlsby, Neil and Giurgiu, Andrei and Jastrzebski, Stanislaw and Morrone, Bruna and De Laroussilhe, Quentin and Gesmundo, Andrea and Attariyan, Mona and Gelly, Sylvain},
  booktitle={International Conference on Machine Learning},
  pages={2790--2799},
  year={2019}
}

@inproceedings{reimers-gurevych-2019-sentence,
    title = "Sentence-{BERT}: Sentence Embeddings using {S}iamese {BERT}-Networks",
    author = "Reimers, Nils  and
      Gurevych, Iryna",
    booktitle = "Proceedings of the 2019 EMNLP-IJCNLP",
    month = nov,
    year = "2019",
    url = "https://aclanthology.org/D19-1410",
    doi = "10.18653/v1/D19-1410",
    pages = "3982--3992",
    abstract = "BERT (Devlin et al., 2018) and RoBERTa (Liu et al., 2019) has set a new state-of-the-art performance on sentence-pair regression tasks like semantic textual similarity (STS). However, it requires that both sentences are fed into the network, which causes a massive computational overhead: Finding the most similar pair in a collection of 10,000 sentences requires about 50 million inference computations ({\textasciitilde}65 hours) with BERT. The construction of BERT makes it unsuitable for semantic similarity search as well as for unsupervised tasks like clustering. In this publication, we present Sentence-BERT (SBERT), a modification of the pretrained BERT network that use siamese and triplet network structures to derive semantically meaningful sentence embeddings that can be compared using cosine-similarity. This reduces the effort for finding the most similar pair from 65 hours with BERT / RoBERTa to about 5 seconds with SBERT, while maintaining the accuracy from BERT. We evaluate SBERT and SRoBERTa on common STS tasks and transfer learning tasks, where it outperforms other state-of-the-art sentence embeddings methods.",
}

@inproceedings{li-etal-2020-sentence,
    title = "On the Sentence Embeddings from Pre-trained Language Models",
    author = "Li, Bohan  and
      Zhou, Hao  and
      He, Junxian  and
      Wang, Mingxuan  and
      Yang, Yiming  and
      Li, Lei",
    booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)",
    month = nov,
    year = "2020",
    url = "https://aclanthology.org/2020.emnlp-main.733",
    doi = "10.18653/v1/2020.emnlp-main.733",
    pages = "9119--9130",
    abstract = "Pre-trained contextual representations like BERT have achieved great success in natural language processing. However, the sentence embeddings from the pre-trained language models without fine-tuning have been found to poorly capture semantic meaning of sentences. In this paper, we argue that the semantic information in the BERT embeddings is not fully exploited. We first reveal the theoretical connection between the masked language model pre-training objective and the semantic similarity task theoretically, and then analyze the BERT sentence embeddings empirically. We find that BERT always induces a non-smooth anisotropic semantic space of sentences, which harms its performance of semantic similarity. To address this issue, we propose to transform the anisotropic sentence embedding distribution to a smooth and isotropic Gaussian distribution through normalizing flows that are learned with an unsupervised objective. Experimental results show that our proposed BERT-flow method obtains significant performance gains over the state-of-the-art sentence embeddings on a variety of semantic textual similarity tasks. The code is available at \url{https://github.com/bohanli/BERT-flow}.",
}

